CONQUER: Context-Aware Representation with Query Enhancement for Text-Based Person Search

Text-Based Person Search (TBPS) aims to retrieve pedestrian images from large galleries using natural language descriptions. This task, essential for public safety applications, is hindered by cross-modal discrepancies and ambiguous user queries. We introduce CONQUER, a two-stage framework designed to address these challenges by enhancing cross-modal alignment during training and adaptively refining queries at inference. During training, CONQUER employs multi-granularity encoding, complementary pair mining, and context-guided optimal matching based on Optimal Transport to learn robust embeddings. At inference, a plug-and-play query enhancement module refines vague or incomplete queries via anchor selection and attribute-driven enrichment, without requiring retraining of the backbone. Extensive experiments on CUHK-PEDES, ICFG-PEDES, and RSTPReid demonstrate that CONQUER consistently outperforms strong baselines in both Rank-1 accuracy and mAP, yielding notable improvements in cross-domain and incomplete-query scenarios. These results highlight CONQUER as a practical and effective solution for real-world TBPS deployment. Source code is available at https://github.com/zqxie77/CONQUER.

==> ICFG.tex <==


\begin{table}[h]
\centering

\caption{Performance comparisons on the ICFG-PEDES dataset. The best results are in \textbf{bold}. }
\resizebox{1 \linewidth}{!}{

\begin{tabular}{l|ccccc}
\toprule[1pt] 
Methods    & R-1 & R-5 & R-10 & mAP   & mINP \\\midrule
% Dual Path~\cite{zheng2020dual} & 38.99  & 59.44  & 68.41   & -     & -    \\
% CMPM/C~\cite{zhang2018deep}    & 43.51  & 65.44  & 74.26   & -     & -    \\
% ViTAA~\cite{wang2020vitaa}     & 50.98  & 68.79  & 75.78   & -     & -    \\
SSAN~\cite{ding2021semantically}      & 54.23  & 72.63  & 79.53   & -     & -    \\
IVT~\cite{shu2022see}       & 56.04  & 73.60  & 80.22   & -     & -    \\
% ISANet~\cite{yan2022image}    & 57.73  & 75.42  & 81.72   & -     & -    \\
CFine~\cite{yan2023clip}     & 60.83  & 76.55  & 82.42   & -     & -    \\
IRRA~\cite{jiang2023cross}      & 63.46  & 80.25  & 85.82   & 38.06 & {7.93} \\
% BiLMa~\cite{fujii2023bilma}  &
% 63.83& 80.15& 85.74& 38.26&-\\
PBSL~\cite{shen2023pedestrian}&57.84 &75.46& 82.15&-&-\\
BEAT\cite{ma2023beat}&58.25& 75.92 &81.96&-&-\\
LCR$^2$S~\cite{yan2023learning}&57.93 &76.08& 82.40 &38.21&-\\
DCEL~\cite{li2023dcel}&64.88& 81.34 &86.72&-&-\\
UniPT~\cite{shao2023unified}&60.09 &76.19&-&-&-\\
    
% RaSa~\cite{bai2023rasa}&   65.28&    80.40 &   85.12 &   41.29&-\\
TBPS~\cite{cao2024empirical}&65.05& 80.34 &85.47& 39.83&-\\
CFAM ~\cite{zuo2024ufinebench}&65.38& 81.17&-&39.42&-\\
OCDL ~\cite{li2025object}&64.53& 80.23&-& 40.76&-\\


  
\midrule

\textbf{CONQUER(Ours)} &\textbf{ 67.70 }& \textbf{81.88}& \textbf{86.98 }& \textbf{40.36} &\textbf{7.82} \\

\bottomrule[1pt]
\end{tabular}}
  \label{tab:icfg}
\end{table}



==> RSTP.tex <==
x x
\bx x x xegin{table}[h]
\centering 

\caption{\textbf{Performance Comparison on the RSTPReid Dataset.} The best results are highlighted in \textbf{bold}, while the second-best results are underlined.}
\resizebox{1 \linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule[1pt] 
Methods & R-1& R-5 & R-10& mAP   & mINP  \\\midrule
% DSSL~\cite{zhu2021dssl}   & 39.05& 62.60  & 73.95& -     & -     \\
SSAN~\cite{ding2021semantically}   & 43.50& 67.80  & 77.15& -     & -     \\
% LBUL~\cite{wang2022look}   & 45.55& 68.20  & 77.85& -     & -     \\
IVT~\cite{shu2022see}    & 46.70& 70.00  & 78.80& -     & -     \\
CFine~\cite{yan2023clip}  & 50.55& 72.50  & 81.60& -     & -     \\
IRRA~\cite{jiang2023cross}  & 60.20 & 81.30  & 88.20 & 47.17 & 25.28 \\ 
% BiLMA~\cite{fujii2023bilma}&61.20& 81.50& 88.80 &48.51&-\\
PBSL~\cite{shen2023pedestrian}&47.80& 71.40& 79.90&-&-\\
BEAT\cite{ma2023beat}&48.10 &73.10 &81.30&-&-\\
LCR$^2$S~\cite{yan2023learning}&54.95& 76.65& 84.70 &40.92&-\\
DCEL~\cite{li2023dcel}& 61.35& 83.95 &{90.45}&-&-\\
    RaSa~\cite{bai2023rasa}&  \underline{ 66.90} &   \underline{ 86.50 } &  \underline{  91.35 }&  \underline{  52.31}&-\\
TBPS~\cite{cao2024empirical} &61.95& 83.55& 88.75& 48.26&-\\
CFAM ~\cite{zuo2024ufinebench}&62.45& 83.55&-&49.50&-\\


OCDL ~\cite{li2025object}&61.60&82.35&-& 49.77&-\\


\midrule
\textbf{CONQUER(Ours)} &\textbf{68.40 }& \textbf{82.95} &\textbf{ 88.85}& \textbf{51.73}& \textbf{28.38 } \\

\bottomrule[1pt]


\end{tabular}}
  \label{tab:rstp}
\end{table}


==> itr_res.tex <==
\begin{table*}[t]
% \caption{Performance Evaluation on Image-Text Retrieval. Bold: best results, Underline: second best results.}
\caption{Performance comparisons on the CUHK-PEDES dataset. The best results are in \textbf{bold}.} 
  \label{tab:1}
\begin{center}
\resizebox{1\textwidth}{0.25\textheight}{ 
\begin{tabular}{l|lcc|ccccc}\toprule[1pt] 
Methods            & Ref.      & Image Enc. & Text Enc.    & R-1 & R-5 & R-10 & mAP   & mINP  \\\midrule
% CMPM/C~\cite{zhang2018deep}& ECCV'18   & RN50       & LSTM         & 49.37  & -      & 79.27   & -     & -     \\
% TIMAM~\cite{sarafianos2019adversarial}              & ICCV'19   & RN101      & BERT         & 54.51  & 77.56  & 79.27   & -     & -     \\
% ViTAA~\cite{wang2020vitaa}              & ECCV'20   & RN50       & LSTM         & 54.92  & 75.18  & 82.90   & 51.60 & -     \\

% DSSL~\cite{zhu2021dssl}               & ACMMM'21     & RN50       & BERT         & 59.98  & 80.41  & 87.56   & -     & -     \\
% SSAN~\cite{ding2021semantically}               & arXiv'21  & RN50       & LSTM         & 61.37  & 80.15  & 86.73   &       & -     \\
% Lapscore~\cite{wu2021lapscore}           & ICCV'21   & RN50       & BERT         & 63.40   & -      & 87.80   & -     & -     \\
% ISANet~\cite{yan2022image}             & arXiv'22  & RN50       & LSTM         & 63.92  & 82.15  & 87.69   & -     & -     \\

% Han et al. ~\cite{han2021text} & BMVC'21   & CLIP-RN101 & CLIP-Xformer & 64.08  & 81.73  & 88.19   & 60.08 & -     \\
% SAF~\cite{li2022learning}                & ICASSP'22 & ViT-Base   & BERT         & 64.13  & 82.62  & 88.40   & -     & -     \\
LBUL~\cite{wang2022look}               & ACMMM'22     & RN50       & BERT         & 64.04  & 82.66  & 87.22   & -     & -     \\
CAIBC~\cite{wang2022caibc}              & ACMMM'22     & RN50       & BERT         & 64.43  & 82.87  & 88.37   & -     & -     \\
AXM-Net~\cite{farooq2022axm}            & ACMMM'22     & RN50       & BERT         & 64.44  & 80.52  & 86.77   & 58.73 & -     \\
LGUR~\cite{shao2022learning}               & ACMMM'22     & DeiT-Small & BERT         & 65.25  & 83.12  & 89.00   & -     & -     \\
DCEL~\cite{qin2022deepdecl}&ACMMM'22&CLIP-ViT& CLIP-Xformer &   71.36&  {88.11}&  {92.48}& 64.25& 48.26\\
IVT~\cite{shu2022see}                & ECCVW'22  & ViT-Base   & BERT         & 65.59  & 83.11  & 89.21   & -     & -     \\
CFine~\cite{yan2023clip}              & TIP'23  & CLIP-ViT   & BERT         & 69.57  & 85.93  & 91.15   & -     & -     \\
IRRA~\cite{jiang2023cross}               & CVPR'23   & CLIP-ViT   & CLIP-Xformer & 73.38  & 89.93  & 93.71   & 66.13 & 50.24 \\
% \textbf{Our RDE-BGE}&-&CLIP-ViT&CLIP-Xformer&74.20&89.57&93.49&66.12&49.62 \\
% \textbf{Our RDE-TGE}&-&CLIP-ViT&CLIP-Xformer&74.85&89.80&93.96&67.23&51.25 \\

% BiLMa~\cite{fujii2023bilma}    & ICCV'23   & CLIP-ViT   & CLIP-Xformer  &74.03& 89.59& 93.62 &66.57&-\\ 

% PBSL~\cite{shen2023pedestrian}&ACMMM'23 & RN50&BERT&65.32 &83.81 &89.26&-&-\\
BEAT\cite{ma2023beat}&ACMMM'23&RN101&BERT& 65.61& 83.45&89.54&-&-\\ 
LCR$^2$S~\cite{yan2023learning}&ACMMM'23&RN50&TextCNN&67.36& 84.19& 89.62& 59.24&\\
DCEL~\cite{li2023dcel}&ACMMM'23&CLIP-ViT& CLIP-Xformer &   75.02&  {90.89}&  {94.52}& -& -\\
APTM~\cite{yang2023towards}&ACMMM'23&Swin-Transformer& Bert &76.53	&90.04	&94.15	&66.91\\
UniPT~\cite{shao2023unified}&ICCV'23&CLIP-ViT& CLIP-Xformer &68.50& 84.67 &-&-&-\\ 

 % RaSa~\cite{bai2023rasa}& IJCAI'23& ALBEFF& ALBEFF&76.51& 90.29 & 94.25 &69.38&\\
% SEN-XL ~\cite{liu2025textsen}& Neural Networks'25&CLIP-ViT& CLIP-Xformer &76.64& 91.33 & 94.66 &69.19& 53.88 \\
TBPS~\cite{cao2024empirical}&AAAI'24&CLIP-ViT& CLIP-Xformer&73.54& 88.19 &92.35& 65.38&-\\
DP~\cite{song2024diverse} & AAAI'24 & CLIP-ViT & CLIP-Xformer & 75.66 & 90.59 & 94.07 & 66.58 & - \\

% IRRA+IRLT~\cite{liu2024causality} & AAAI'24 & CLIP-ViT & CLIP-Xformer & 74.46 & 90.19 & 94.01 & - & - \\
UASA~\cite{zhao2024unifying} & AAAI'24 & CLIP-ViT & CLIP-Xformer & 74.25 & 89.83 &  93.58 & 66.15 & - \\

{RDE}~\cite{qin2024noisy} & CVPR'24 & CLIP-ViT& CLIP-Xformer & {75.94} &{90.14}& {94.12} &{67.56}& {51.44} \\  

CFAM ~\cite{zuo2024ufinebench}&CVPR'24&CLIP-ViT& CLIP-Xformer&75.60& 90.53&-&67.27&-\\
% MLLM+IRRA ~\cite{tan2024harnessingmllm}&CVPR'24&CLIP-ViT& CLIP-Xformer&76.82&  91.16&-&69.55&-\\
MGRL ~\cite{lv2024mgrl}&ICASSP'24&CLIP-ViT& CLIP-Xformer&73.91& 90.68&-& 67.28&-\\
DM-Adapter~\cite{liu2025dm} & AAAI'25 & CLIP-ViT & CLIP-Xformer & 72.17 & 88.74 & 92.85 &64.33 & - \\

OCDL ~\cite{li2025object}&ICASSP'25&CLIP-ViT& CLIP-Xformer&75.10& 89.43&-& 68.18&-\\
\midrule


\textbf{CONQUER (Ours) }& -& CLIP-ViT& CLIP-Xformer & \textbf{77.13} & \textbf{90.06}&\textbf {93.89} &\textbf{68.75}& \textbf{ 53.01 } \\  
\bottomrule[1pt]
\end{tabular}}
% \caption{Performance comparisons on the CUHK-PEDES dataset. The best results are in \textbf{bold}.} 

\end{center}
\end{table*}


